Observability of Hypergraphs

In this paper we develop a framework to study observability for uniform hypergraphs. Hypergraphs, being extensions of graphs, allow edges to connect multiple nodes and unambiguously represent multi-way relationships which are ubiquitous in many real-world networks. We extend the canonical homogeneous polynomial or multilinear dynamical system on uniform hypergraphs to include linear outputs, and we derive a Kalman-rank-like condition for assessing the local weak observability. We propose an exact techniques for determining the local observability criterion, and we propose a greedy heuristic to determine the minimum set of observable nodes. Numerical experiments demonstrate our approach on several hypergraph topologies and a hypergraph representations of neural networks within the mouse hypothalamus.

==> colors.tex <==
\definecolor{aureolin}{rgb}{0.99, 0.93, 0.0}
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\definecolor{capri}{rgb}{0.0, 0.75, 1.0}
\definecolor{darkpink}{rgb}{0.91, 0.33, 0.5}
\definecolor{eggplant}{rgb}{0.38, 0.25, 0.32}
\definecolor{fuchsia}{rgb}{1.0, 0.0, 1.0}
\definecolor{goldenrod}{rgb}{0.85, 0.65, 0.13}
\definecolor{green(pigment)}{rgb}{0.0, 0.65, 0.31}
\definecolor{salmon}{rgb}{1.0, 0.55, 0.41}
\definecolor{amber}{rgb}{1.0, 0.75, 0.0}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{ashgrey}{rgb}{0.7, 0.75, 0.71}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}
\definecolor{blue-green}{rgb}{0.0, 0.87, 0.87}
\definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
\definecolor{brilliantrose}{rgb}{1.0, 0.33, 0.64}
\definecolor{emerald}{rgb}{0.31, 0.78, 0.47}
\definecolor{sandstorm}{rgb}{0.93, 0.84, 0.25}
\definecolor{teal}{rgb}{0.0, 0.5, 0.5}
\definecolor{sealbrown}{rgb}{0.2, 0.08, 0.08}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\newcommand\redpt[1]{\fill[black] (#1) circle[radius=1mm];}
